Listening to Sounds of Silence for Speech Denoising

We introduce a deep learning model for speech denoising, a long-standing challenge in audio analysis arising in numerous applications. Our approach is based on a key observation about human speech: there is often a short pause between each sentence or word. In a recorded speech signal, those pauses introduce a series of time periods during which only noise is present. We leverage these incidental silent intervals to learn a model for automatic speech denoising given only mono-channel audio. Detected silent intervals over time expose not just pure noise but its time-varying features, allowing the model to learn noise dynamics and suppress it from the speech signal. Experiments on multiple datasets confirm the pivotal role of silent interval detection for speech denoising, and our method outperforms several state-of-the-art denoising methods, including those that accept only audio input (like ours) and those that denoise based on audiovisual input (and hence require more information). We also show that our method enjoys excellent generalization properties, such as denoising spoken languages not seen during training.

==> Makefile <==
# name of latex document
MAINDOC := 0_Main

# latex source file
TEXSRC := $(wildcard *.tex)
BIBSRC := $(wildcard *.bib)

ifneq ($(strip $(BIBSRC)),)
BBLSRC := $(MAINDOC).bbl
endif

# latex program
TEX      := latex
PDFLATEX := pdflatex
BIB      := bibtex

# flags
TEX_FLAGS :=
PDF_FLAGS :=
BIB_FLAGS :=

#=====================================================#
# Display Codes (this is so we can track passes)
#=====================================================#
MOVE_TO_COL	= @echo  "\\033[60G"
SETCOLOR_RED 	= @echo  "\\033[0;31m"
SETCOLOR_GREEN 	= @echo  "\\033[0;32m"
SETCOLOR_BLUE	= @echo  "\\033[0;34m"
SETCOLOR_BACK	= @echo  "\\033[0m"

all: $(MAINDOC).pdf

pdf: $(MAINDOC).pdf

dvi: $(MAINDOC).dvi

full: $(BBLSRC) $(TEXSRC)
	@$(PDFLATEX) $(PDF_FLAGS) $(MAINDOC)
	$(SETCOLOR_GREEN)
	@echo "=========================FINAL PASS=============================="
	$(SETCOLOR_BACK)
	@$(PDFLATEX) $(PDF_FLAGS) $(MAINDOC)


%.dvi : %.aux
	$(SETCOLOR_BLUE)
	@echo "=========================AUX -> DVI PASS=============================="
	$(SETCOLOR_BACK)
	@$(TEX) $(TEX_FLAGS) $(*F)
	
$(MAINDOC).bbl : $(BIBSRC) $(TEXSRC) 
ifneq ($(strip $(BIBSRC)),)
	$(SETCOLOR_GREEN)
	@echo "=========================LaTeX PASS=============================="
	$(SETCOLOR_BACK)
	$(PDFLATEX) $(TEX_FLAGS) $(MAINDOC)
	$(SETCOLOR_GREEN)
	@echo "=========================BibTex PASS=============================="
	$(SETCOLOR_BACK)
	@$(BIB) $(BIB_FLAGS) $(MAINDOC)
endif

$(MAINDOC).pdf : $(TEXSRC)
	$(SETCOLOR_GREEN)
	@echo "=========================SINGLE PASS=============================="
	$(SETCOLOR_BACK)
	@$(PDFLATEX) $(PDF_FLAGS) $(MAINDOC)

.PHONY: all clean

clean:
	-$(RM) *.aux *.pdf *.bbl *.blg *.log

